Robust dynamic self-triggered control for nonlinear systems using hybrid Lyapunov functions

Self-triggered control (STC) is a resource efficient approach to determine sampling instants for Networked Control Systems. At each sampling instant, an STC mechanism determines not only the control inputs but also the next sampling instant. In this article, an STC framework for perturbed nonlinear systems is proposed. In the framework, a dynamic variable is used in addition to current state information to determine the next sampling instant, rendering the STC mechanism dynamic. Using dynamic variables has proven to be powerful for increasing sampling intervals for the closely related concept of event-triggered control, but has so far not been exploited for STC. Two variants of the dynamic STC framework are presented. The first variant can be used without further knowledge on the disturbance and leads to guarantees on input-to-state stability. The second variant exploits a known disturbance bound to determine sampling instants and guarantees asymptotic stability of a set containing the origin. In both cases, hybrid Lyapunov function techniques are used to derive the respective stability guarantees. Different choices for the dynamics of the dynamic variable, that lead to different particular STC mechanisms, are presented for both variants of the framework. The resulting dynamic STC mechanisms are illustrated with two numerical examples to emphasize their benefits in comparison to existing static STC approaches.

==> proof_theo_fir_lp.tex <==
%
\subsubsection{Proof of Corollary~\ref{theo_fir_lp}}
\label{proof_coro_fir}
%
%
%
%
%
%
%
%
%
%
%
%
	Similar as in the proof of Theorem~\ref{prop_fir}, we obtain that 	
	\begin{equation}
	\label{eq_fir_iss_res_gain}
	\begin{split}
	V(x(t,j))
	\leq& e^{-\epsilon_\refer t}  \max \left\lbrace V(x(0,0)), \abs{\eta(0,0)} \right\rbrace\\
	&+ \maxvar \int_{0}^{t} e^{- \epsilon_\refer(t-\tau)} \thetavar^p\abs{w}^p d\tau		
	\end{split}
	\end{equation}
	holds for all $(t,j) \in \text{dom}~\xi$.
	
	%
	From Proposition~\ref{prop_hybrid}, we obtain moreover
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	\begin{equation}
	\begin{split}
	\int_{\svar_j}^{t} \norm{z(\tau)}^p d\tau \leq&\maxvart{j}\int_{\svar_j}^{t} e^{ -\epsilon_\ivar{j} (t-\tau)} \norm{z(\tau)}^p d\tau\\
	\leq & \maxvart{j} \left(\vphantom{ \int_{\svar_j}^{t}} e^{ \epsilon_\ivar{j} (t-\svar_j)} V(x(\tvar_j)) - V(x(t,j))\right.\\
	&\left.+  \maxvar\int_{\svar_j}^{t} e^{-\epsilon_\refer (t-\tau)} \theta_1^p \norm{w(\tau)}^p d\tau\right)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             
	\end{split}	 	 
	\end{equation}
	for all $(t,j) \in\text{dom}~\xi$ and $\maxvart{j} = \underset{i \in \left[1,\dots,n_\tpar\right]}{\max} \frac{1}{\min\left\lbrace e^{ -\epsilon_i T_{\max} (\gamma_i,L-\frac{\epsilon_i}{2})},1 \right\rbrace}$, where we used that $V(x(t,j)) \leq U(\xi(t,j))$. 
	
	
	Thus, for $\svar_{\barj} \leq t \leq \svar_{\barj+1}$ for any $\barj \in \mathbb{N}_0$, we have that 
	\begin{equation}
	\label{eq_fir_l21}
	\begin{split}
	&\int_{0}^{t} \norm{z(\tau)}^p d\tau = \int_{\svar_{\bar j}}^{t}  \norm{z(\tau)}^p d\tau+ \sum_{j = 0}^{\bar j -1}  \int_{\svar_j}^{\svar_{j+1}}  \norm{z(\tau)}^p d\tau \\
	\leq &\maxvart{}\left( e^{ -\epsilon_\ivar{\barj} (t-\svar_{\bar j})} V(x(\tvar_{\bar j})) - V(x(t,\bar j)) \vphantom{\int_{\svar_j}^{\svar_{j+1}}}\right.\\ 
	&+  \maxvar \int_{\svar_{\bar j}}^{t} e^{-\epsilon_\refer (t-\tau)} \theta_1^p \norm{w(\tau)}^p d\tau   \\
	&+\sum_{j = 0}^{\bar j -1} e^{ -\epsilon_\ivar{j} (\svar_{j+1}-\svar_j)} V(\xi(\tvar_j)) - V(x(s_{j+1}))\\ %
	&\left.+ \maxvar\sum_{j = 0}^{\barj -1}  \int_{\svar_j}^{\svar_{j+1}} e^{-\epsilon_\refer(\svar_{j+1}-\tau)} \theta_1^p \norm{w(\tau)}^p d\tau\right)\\
	\leq&\maxvart{} \left(\sum_{j = 1}^{\bar j } \left(e^{-\epsilon_\ivar{j} (\svar_{j+1}-\svar_j)}-1\right) V(x(\tvar_j))\right. %
	\\
	&\left.+ e^{-\epsilon_\ivar{1} (\svar_{1}-\svar_0)} V(x(\tvar_0)) +\maxvar  \int_{0}^{t}  \theta_1^p \norm{w(\tau)}^p d\tau\vphantom{\sum_{j = 0}^{\barj -1}}\right).
	\end{split}		
	\end{equation}
	Using \eqref{eq_fir_iss_res_gain} we obtain for $k_3 = \max\left\lbrace\left(\underset{i}{\max} e^{-\epsilon_i t_{\max}}-1\right),0\right\rbrace$
	\begin{equation}
	\label{eq_fir_V_est}
	\begin{split}
	&\sum_{j = 1}^{\barj -1} \left(e^{  -\epsilon_\ivar{j} (\svar_{j+1}-\svar_j)} -1\right)V(x(\tvar_j)) \\
	\leq &  k_3 \sum_{j = 1}^{\bar j -1} V(x(\tvar_j))  \\
	\overset{\eqref{eq_fir_iss_res_gain}}{\leq} & k_3 \sum_{j = 1}^{\bar j -1} e^{-\epsilon_\refer \svar_{j}} V(x(0)) \\
	&+ k_3 \maxvar \sum_{j = 1}^{\bar j -1} \int_{t_0}^{\svar_j} e^{-\epsilon_\refer(\svar_j-\tau)} \theta^p_1 \norm{w(\tau)}^p d\tau.
	\end{split}
	\end{equation}
%
%
%
%
%
%
%
%
%
%
	\MH{Do we implicitly assume here that $\epsilon_i < 0$ for some $i$?}
	Note that 
	\begin{equation}
	\label{eq_fir_geo_V}
	\sum_{j = 1}^{\bar j -1} e^{-\epsilon_\refer \svar_{j}} V(x(\tvar_0)) \leq \frac{ V(x(\tvar_0))}{1-e^{-\epsilon_\refer t_{\min}}}.
	\end{equation}
	Moreover, observe that 
	\begin{equation}
	\label{eq_fir_sum_est}
	\begin{split}
	&\sum_{j = 1}^{\bar j -1} \int_{0}^{\svar_j} e^{-\epsilon_\refer(\svar_j-\tau)} \theta^p_1 \norm{w(\tau)}^p d\tau \\ %
	=& \sum_{r = 0}^{\bar j -1} \int_{\svar_r}^{\svar_{r+1}} e^{-\epsilon_\refer(\svar_{r+1}-\tau)} \theta^p_1 \norm{w(\tau)}^p d\tau
	\sum_{q=r}^{\bar{j}-1} e^{-\epsilon_\refer \left(\svar_{q+1} - \svar_{r+1}\right)}\\
	\leq & \sum_{r = 0}^{\bar j -1} \int_{\svar_r}^{\svar_{r+1}} e^{-\epsilon_\refer(\svar_{r+1}-\tau)} \theta^p_1 \norm{w(\tau)}^p d\tau
	\sum_{q=0}^{\bar{j}-1-r} e^{-\epsilon_\refer t_{\min}q}\\
	\leq& \int_{\svar_0}^{\svar_{\bar j}} 
	%
	\theta^p_1 \norm{w(\tau)}^p d\tau \frac{1}{1-e^{-\epsilon_\refer t_{\min}}}.
	\end{split}	
	\end{equation}
	Combining \eqref{eq_fir_l21}, \eqref{eq_fir_V_est},\eqref{eq_fir_geo_V} and \eqref{eq_fir_sum_est}, we obtain
	\begin{equation}
	\begin{split}
	&\int_{0}^{t} \norm{z(\tau)}^p d\tau\\
	\leq &\frac{\maxvart{} k_3}{1-e^{-\epsilon_\refer t_{\min}}} \left( V(x(\tvar_0))\vphantom{\int_{\svar_0}^{\svar_{\bar j}} e^{-\epsilon_\refer(\svar_{r+1}-\tau)} \theta^p_1 \norm{w(\tau)}^p d\tau}
	+\maxvar\int_{\svar_0}^{\svar_{\bar j}} 
	%
	\theta^p_1 \norm{w(\tau)}^p d\tau\right)
	\\
	&+ \maxvart{}e^{  -\epsilon_i (\svar_{j+1}-\svar_j)} V(x(\tvar_0)) +  \maxvart{}\maxvar\int_{\svar_0}^{t}  \theta_1^p \norm{w(\tau)}^p d\tau.
	\end{split}
	\end{equation}
	Note that $\sqrt[p]{a+b} \leq \sqrt[p]{a} + \sqrt[p]{b}$. 
	We can thus conclude that Definition~\ref{def_lp} holds with 
	\begin{equation}
	\begin{split}
	\chi\left(\abs{\begin{bmatrix}
		x(0,0)\\
		e(0,0)\\
		\eta(0,0)
		\end{bmatrix}}\right) =&\left(\frac{ k_3}{1-e^{-\epsilon_\refer t_{\min}}} + \underset{i}{\max} e^{-\epsilon_i t_{\max}}\right)^{\frac{1}{p}}\\ 
	&\cdot \maxvart{}^{\frac{1}{p}}\left(\overline{\alpha}_V(\abs{x(0,0)})\right)^{\frac{1}{p}}
	\end{split}
	\end{equation} 
	and 
	\begin{equation}
	\theta = \maxvart{}^{\frac{1}{p}}\maxvar^{\frac{1}{p}}\left(1+ \frac{ k_3}{1-e^{-\epsilon_\refer t_{\min}}}\right)^{\frac{1}{p}} \theta_1.
	\end{equation} \hfill\hfill\qed
%

==> proof_theo_fir_lp_quan.tex <==
%
\begin{proof}[Proof of Theorem~\ref{theo_fir_lp}]
	Similar as in the proof of Theorem~\ref{prop_fir}, we obtain	for $\svar_{j+1} \leq t \leq \svar_j$ with $\Lambda_\ivar{j} = L_\ivar{j}+\frac{\epsilon_\ivar{j}}{2}$ that 
	\begin{equation}
	\label{eq_V_dec_fir_gain}
	\begin{split}
	&U_\ivar{j}(\xi(t,j+1))	\\
	\leq 	&	e^{ -\epsilon_\ivar{j} (t-\svar_j)}V(\xi(\tvar_j)) + \int_{\svar_j}^{t} e^{ -\epsilon_\ivar{j} (t-\tau)} \theta_{\ivar{j}}^p\abs{w(\tau)}^p d\tau\\
	\leq& e^{ -\epsilon_\ivar{j} (t-\svar_j)}V(\xi(\tvar_j)) \\
	&+ e^{\left(-\epsilon_\ivar{j}+\epsilon_\refer\right) t_{\max}} \int_{\svar_j}^{t} e^{-\epsilon_\refer (t-\tau)} \theta_\ivar{j}^p\abs{w(\tau)}^p d\tau\\
	\overset{\eqref{eq_def_alpha_w}}{\leq}&  e^{ -\epsilon_\ivar{j} (t-\svar_j)}V(\xi(\tvar_j)) +  \int_{\svar_j}^{t}e^{-\epsilon_\refer (t-\tau)} \thetavar\abs{w(\tau)} d\tau,
	\end{split}
	\end{equation}
	where $U_\ivar{j}(\xi)$ is the function according to \eqref{eq_def_u} for the parameters $\gamma_\ivar{j}$ and $\Lambda_\ivar{j}$. Using similar steps as in the proof of Theorem~\ref{prop_fir}, we obtain that 	
	\begin{equation}
	\label{eq_fir_iss_res_gain}
	\begin{split}
	V(x(t,j))
	\leq& e^{-\epsilon_\refer t}  \max \left\lbrace V(x(0,0)), \abs{\eta(0,0)} \right\rbrace\\
	&+  \int_{0}^{t} e^{- \epsilon_\refer(t-\tau)} \thetavar^p\abs{w}^p d\tau		
	\end{split}
	\end{equation}
	holds for all $(t,j)$.
	
	%
	From Proposition~\ref{prop_hybrid}, we obtain moreover
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	\begin{equation}
	\begin{split}
	\int_{\svar_j}^{t} \norm{z(\tau)}^p d\tau \leq&\maxvart{j}\int_{\svar_j}^{t} e^{ -\epsilon_\ivar{j} (t-\tau)} \norm{z(\tau)}^p d\tau\\
	\leq & \maxvart{j} \left(\vphantom{ \int_{\svar_j}^{t}} e^{ \epsilon_\ivar{j} (t-\svar_j)} V(x(\tvar_j)) - V(x(t,j))\right.\\
	&\left.+  \int_{\svar_j}^{t} e^{-\epsilon_\refer (t-\tau)} \theta_1^p \norm{w(\tau)}^p d\tau,\right) 
	\end{split}	 	 
	\end{equation}
	for all $(t,j)$ and $\maxvart{j} = \underset{i \in \left[1,\dots,n_\tpar\right]}{\max} \frac{1}{\min\left\lbrace e^{ -\epsilon_i T_{\max} (\gamma_i,L-\frac{\epsilon_i}{2})},1 \right\rbrace}$, where we used that $V(x(t,j)) \leq U(\xi(t,j)$. 
	
	
	Thus, for $\svar_{\barj+1} \leq t \leq \svar_{\barj}$ for any $\barj \in \mathbb{N}_0$, we have that 
	\begin{equation}
	\label{eq_fir_l21}
	\begin{split}
	&\int_{0}^{t} \norm{z(\tau)}^p d\tau = \int_{\svar_{\bar j}}^{t}  \norm{z(\tau)}^p d\tau+ \sum_{j = 0}^{\bar j -1}  \int_{\svar_j}^{\svar_{j+1}}  \norm{z(\tau)}^p d\tau \\
	\leq &\maxvart{}\left( e^{ -\epsilon_\ivar{\barj} (t-\svar_{\bar j})} V(x(\tvar_{\bar j})) - V(x(t,\bar j)) \vphantom{\int_{\svar_j}^{\svar_{j+1}}}\right.\\ 
	&+  \int_{\svar_{\bar j}}^{t} e^{-\epsilon_\refer (t-\tau)} \theta_1^p \norm{w(\tau)}^p d\tau   \\
	&+\sum_{j = 0}^{\bar j -1} e^{ -\epsilon_\ivar{j} (\svar_{j+1}-\svar_j)} V(\xi(\tvar_j)) - V(x(s_{j+1}))\\ %
	&\left.+ \sum_{j = 0}^{\barj -1}  \int_{\svar_j}^{\svar_{j+1}} e^{-\epsilon_\refer(\svar_{j+1}-\tau)} \theta_1^p \norm{w(\tau)}^p d\tau\right)\\
	\leq&\maxvart{} \left(\sum_{j = 1}^{\bar j } \left(e^{-\epsilon_\ivar{j} (\svar_{j+1}-\svar_j)}-1\right) V(x(\tvar_j))\right. %
	\\
	&\left.+ e^{-\epsilon_\ivar{j} (\svar_{j+1}-\svar_j)} V(x(\tvar_0)) +  \int_{\svar_0}^{t}  \theta_1^p \norm{w(\tau)}^p d\tau\vphantom{\sum_{j = 0}^{\barj -1}}\right)
	\end{split}		
	\end{equation}
	Using \eqref{eq_fir_iss_res_gain} we obtain
	\begin{equation}
	\label{eq_fir_V_est}
	\begin{split}
	&\sum_{j = 1}^{\barj -1} \left(e^{  -\epsilon_\ivar{j} (\svar_{j+1}-\svar_j)} -1\right)V(x(\tvar_j)) \\
	\leq &  \left(\underset{i}{\max} e^{-\epsilon_i t_{\max}}-1\right) \sum_{j = 1}^{\bar j -1} V(x(\tvar_j))  \\
	\overset{\eqref{eq_fir_iss_res}}{\leq} & \left(\underset{i}{\max} e^{-\epsilon_i t_{\max}}-1\right) \sum_{j = 1}^{\bar j -1} e^{-\epsilon_\refer \svar_{j}} V(x(0)) \\
	&+ \left(\underset{i}{\max} e^{-\epsilon_i t_{\max}}-1\right)\sum_{j = 1}^{\bar j -1} \int_{t_0}^{\svar_j} e^{-\epsilon_\refer(\svar_j-\tau)} \theta^p_1 \norm{w(\tau)}^p d\tau.
	\end{split}
	\end{equation}
	\MH{Do we implicitly assume here that one $\epsilon_i$ is negative?}Note that 
	\begin{equation}
	\label{eq_fir_geo_V}
	\sum_{j = 1}^{\bar j -1} e^{-\epsilon_\refer \svar_{j}} V(x(\tvar_0)) \leq \frac{ V(x(\tvar_0))}{1-e^{-\epsilon_\refer t_{\min}}}.
	\end{equation}
	Moreover, observe that 
	\begin{equation}
	\label{eq_fir_sum_est}
	\begin{split}
	&\sum_{j = 1}^{\bar j -1} \int_{0}^{\svar_j} e^{-\epsilon_\refer(\svar_j-\tau)} \theta^p_1 \norm{w(\tau)}^p d\tau \\ %
	=& \sum_{r = 0}^{\bar j -1} \int_{\svar_r}^{\svar_{r+1}} e^{-\epsilon_\refer(\svar_{r+1}-\tau)} \theta^p_1 \norm{w(\tau)}^p d\tau
	\sum_{q=r}^{\bar{j}-1} e^{-\epsilon_\refer \left(\svar_{q+1} - \svar_{r+1}\right)}\\
	\leq & \sum_{r = 0}^{\bar j -1} \int_{\svar_r}^{\svar_{r+1}} e^{-\epsilon_\refer(\svar_{r+1}-\tau)} \theta^p_1 \norm{w(\tau)}^p d\tau
	\sum_{q=0}^{\bar{j}-1-r} e^{-\epsilon_\refer t_{\min}q}\\
	\leq& \int_{\svar_0}^{\svar_{\bar j}} 
	%
	\theta^p_1 \norm{w(\tau)}^p d\tau \frac{1}{1-e^{-\epsilon_\refer t_{\min}}}
	\end{split}	
	\end{equation}
	Combining \eqref{eq_fir_l21}, \eqref{eq_fir_V_est},\eqref{eq_fir_geo_V} and \eqref{eq_fir_sum_est}, we obtain
	\begin{equation}
	\begin{split}
	&\int_{0}^{t} \norm{z(\tau)}^p d\tau\\
	\leq &\maxvart{}\frac{ \left(\underset{i}{\max} e^{-\epsilon_i t_{\max}}-1\right)}{1-e^{-\epsilon_\refer t_{\min}}} \left( V(x(\tvar_0))\vphantom{\int_{\svar_0}^{\svar_{\bar j}} e^{-\epsilon_\refer(\svar_{r+1}-\tau)} \theta^p_1 \norm{w(\tau)}^p d\tau}
	+\int_{\svar_0}^{\svar_{\bar j}} 
	%
	\theta^p_1 \norm{w(\tau)}^p d\tau\right)
	\\
	&+ \maxvart{}e^{  -\epsilon_i (\svar_{j+1}-\svar_j)} V(x(\tvar_0)) +  \maxvart{}\int_{\svar_0}^{t}  \theta_1^p \norm{w(\tau)}^p d\tau.
	\end{split}
	\end{equation}
	Note that $\sqrt[p]{a+b} \leq \sqrt[p]{a} + \sqrt[p]{b}$. 
	We can thus conclude that Definition~\ref{def_lp} holds with 
	\begin{equation}
	\begin{split}
	S(\cdot) =&\left(\frac{ \left(\underset{i}{\max} e^{-\epsilon_i t_{\max}}-1\right)}{1-e^{-\epsilon_\refer t_{\min}}} + \underset{i}{\max} e^{-\epsilon_i t_{\max}}\right)^{\frac{1}{p}}\\ 
	&\cdot \maxvart{}^{\frac{1}{p}}\left(\overline{\alpha}_V(\norm{x(\tvar_0)})\right)^{\frac{1}{p}}
	\end{split}
	\end{equation} 
	and 
	\begin{equation}
	\theta = \maxvart{}^{\frac{1}{p}}\left(1+ \frac{ \left(\underset{i}{\max} e^{-\epsilon_i t_{\max}}-1\right)}{1-e^{-\epsilon_\refer t_{\min}}}\right)^{\frac{1}{p}} \theta_1.
	\end{equation}
\end{proof}

==> proof_theo_iir_loc.tex <==
%
\subsubsection{Proof of Theorem~\ref{theo_iir_loc}}
\label{proof_theo_iir_loc}
		Similar as in the proof of Theorem~\ref{prop_fir}, we obtain that 		
		$t_{\min} \leq \svar_{j+1} - \svar_j \leq t_{\max} \coloneqq \underset{i \in \left[1,\dots,n_\tpar\right]}{\max} \delta T_{\max}\left(\gamma_i,L_i+\frac{\epsilon_i}{2}\right)
		$ holds.
%
		Suppose that $x(\tvar_0) \in \mathcal{X}$.
		
		Now, we will show by induction that 
		\begin{equation}
		\label{eq_iir_loc_ind}
		\begin{split}
		&V(x(t,j)) \\
		\leq& \min \left\lbrace c_w + e^{-\bar\epsilon t} \max \left\lbrace V(x(0,0)),\abs{\eta(0,0)} \right\rbrace, c_{\max} \right\rbrace
		\end{split}
		\end{equation}
		and
		\begin{equation}
		\label{eq_iir_loc_ind_eta}
		\begin{split}
		&\eta(t,j) \\
		\leq& \min \left\lbrace c_w + e^{-\bar\epsilon t} \max \left\lbrace V(x(0,0)),\abs{\eta(0,0)} \right\rbrace, c_{\max} \right\rbrace
		\end{split}
		\end{equation}
		hold for all $(t,j) \in \text{dom}~\xi$ and $\bar \epsilon = \min\left\lbrace \epsilon_1,\epsilon_\refer\right\rbrace$. Both inequalities trivially hold for $t = j = 0$. Now suppose they holds for all $\tvar_j$ with $j \leq \barj$ for some $\barj \in \mathbb{N}$. 
		
		Plugging \eqref{eq_iir_loc_ind} and \eqref{eq_iir_loc_ind_eta} for $(t,j) = \tvar_\barj$ into \eqref{eq_S_iir}, we obtain for $\svar_\barj\leq t \leq \svar_{\barj+1}$ since $r_1+r_2 \leq 1$ that 
		\begin{equation}
			\begin{split}
				&\eta(t,\barj+1) = S(\eta(\tvar_\barj),x(\tvar_\barj))\\
				\leq& \min \left\lbrace c_w + e^{-\bar\epsilon \svar_{\barj+1}} \max \left\lbrace V(x(0,0)),\abs{\eta(0,0)} \right\rbrace, c_{\max} \right\rbrace
			\end{split}		
		\end{equation}
		\MH{provide here intermediate step?}
		and thus that \eqref{eq_iir_loc_ind_eta} holds also for $\svar_\barj \leq t \leq\svar_{\barj+1}$ and $\barj+1$. 
		
		
		%
		%
		
		Further, we can conclude from the modified version of Algorithm~\ref{algo_trig_window} that either \eqref{eq_dec_gen_loc} and \eqref{eq_bound_aux_loc} hold for $\barj$, some $\ivar{\barj}\in\left\lbrace 2,\dots,n_\tpar\right\rbrace$\MH{Is this the better way to write the set?} and $\svar_\barj \leq t \leq \svar_{\barj+1}$ or that $\svar_{\barj+1} = \svar_{\barj} + T_{\max}(\gamma_1,L_1+\frac{\epsilon_1}{2})$.
		
		In the former case, \eqref{eq_dec_gen_loc} implies since $C(x(\tvar_j),\eta(\tvar_j)) \leq c_{\max}$ that \eqref{eq_bound_U_loc} holds for $\barj$ with $\epsilon = \epsilon_{i_\barj}$. Thus, it follows in this case from Proposition~\ref{prop_hybrid_loc} and the modified version of Algorithm~\ref{algo_trig_window} that \eqref{eq_cond_dec} holds for $\barj$ and $\svar_\barj \leq t \leq \svar_{\barj+1}$. Similar as in the proof of Theorem~\ref{theo_iir}, we obtain due to the definition of $C(\eta,x)$ according to \eqref{eq_iir_C_loc} with \eqref{eq_iir_loc_ind} and \eqref{eq_iir_loc_ind_eta} for $(t,j) = \tvar_j$ with $j \leq \barj$ that 
		\begin{equation}
		\label{eq_iir_loc_C}
		\begin{split}
		&C(x(\tvar_\barj),\eta(\tvar_\barj))\\
		\leq& \min \left\lbrace c_w + e^{-\bar\epsilon \svar_\barj} \max \left\lbrace V(x(0,0)),\abs{\eta(0,0)} \right\rbrace, c_{\max} \right\rbrace.
		\end{split}
		\end{equation}
		Plugging \eqref{eq_iir_loc_C} in \eqref{eq_cond_dec}, we can conclude that \eqref{eq_iir_loc_ind} holds in this case for $\barj+1$ and $\svar_\barj \leq t \leq \svar_{\barj+1}$.
		
		In the other case, i.e., if $\svar_{\barj+1} = \svar_{\barj} + T_{\max}(\gamma_1,L_1+\frac{\epsilon_1}{2})$, we observe that \eqref{eq_bound_U_loc} holds for $\epsilon = \epsilon_1$ since $V(x(\tvar_\barj)) \leq c_{\max}$, $\frac{\alpha_w\left(\abs{\bar w}\right)}{\epsilon} \leq c_w \leq c_{\max}$ and $e^{-\epsilon_1 \auxvar(\tvar_\barj^+)} \leq 1$. Thus, we can use in this case Proposition~\ref{prop_hybrid_loc} and obtain that 
		\begin{equation}
		\label{eq_iir_eps1_loc}
		\begin{split}
		V(x(t,\barj+1)) 
		\leq&	e^{ -\epsilon_1 (t-\svar_\barj)}V(x(\tvar_\barj))\\
		& + \frac{\alpha_w\left(\abs{\bar w}\right)}{\epsilon_1} \left(1-e^{-\epsilon_1(t-\svar_\barj)}\right)
		\end{split}
		\end{equation} 
		\MH{Note that this is identical to \eqref{eq_fir_eps1_loc}.}
		holds for $\svar_\barj \leq t \leq \svar_{\barj+1}$. Plugging \eqref{eq_iir_loc_ind} for $(t,j) = \tvar_\barj$ into \eqref{eq_iir_eps1_loc}, we obtain 
		\begin{equation}
		\begin{split}
		&V(x(t,\barj+1))\\ 
		\leq&	e^{ -\epsilon_1 (t-\svar_\barj)}\min \left\lbrace c_w + e^{-\bar\epsilon \svar_\barj} \max \left\lbrace V(x(0,0)),\abs{\eta(0,0)} \right\rbrace, c_{\max} \right\rbrace\\
		&+ \frac{\alpha_w\left(\abs{\bar w}\right)}{\epsilon_1} \left(1-e^{-\epsilon_1(t-\svar_\barj)}\right)\\
		\leq& e^{ -\epsilon_1 (t-\svar_\barj)}\min \left\lbrace c_w + e^{-\bar\epsilon \svar_\barj} \max \left\lbrace V(x(0,0)),\abs{\eta(0,0)} \right\rbrace, c_{\max} \right\rbrace\\
		&+ c_w \left(1-e^{-\epsilon_1(t-\svar_\barj)}\right)\\
		\leq& \min \left\lbrace c_w + e^{-\bar\epsilon t} \max \left\lbrace V(x(0,0)),\abs{\eta(0,0)} \right\rbrace, c_{\max} \right\rbrace
		\end{split}
		\end{equation}
		\MH{Seems this violates the page margin...}
		for $\svar_\barj\leq t \leq \svar_{\barj+1}$. Thus \eqref{eq_iir_loc_ind} holds in both cases  also for $\tvar_{\barj+1}$ and hence by induction for all $(t,j) \in\text{dom}~\xi$. RAS of $\mathcal{R}$ follows immediately from \eqref{eq_iir_loc_ind} and $t \geq \frac{t+j t_{\min}}{2}$ with 
		\begin{equation*}
		\begin{split}
		&\beta\left(\abs{\begin{bmatrix}
			x(0,0)\\
			e(0,0)\\
			\eta(0,0)
			\end{bmatrix}},t, j\right)\\
		=& e^{-\bar \epsilon \left(\frac{t+jt_{\min}}{2}\right)} \max \left\lbrace \overline{\alpha}_V \abs{\begin{bmatrix}
			x(0,0)\\
			e(0,0)\\
			\eta(0,0)
			\end{bmatrix}}, \abs{\begin{bmatrix}
			x(0,0)\\
			e(0,0)\\
			\eta(0,0)
			\end{bmatrix}} \right\rbrace.
		\end{split}			 	
		\end{equation*}
		\MH{Omit this proof since it is similar to the proof of Theorem~\ref{prop_fir_loc}?}
	\hfill\hfill\qed

==> proof_theo_ref_loc.tex <==
\subsubsection{Proof of Theorem~\ref{theo_ref_loc}}
\label{proof_theo_ref_loc}
	Similar as in the proof of Theorem~\ref{prop_fir}, we obtain that 		
	$t_{\min} \leq \svar_{j+1} - \svar_j \leq t_{\max} \coloneqq \underset{i \in \left[1,\dots,n_\tpar\right]}{\max} \delta T_{\max}\left(\gamma_i,L_i+\frac{\epsilon_i}{2}\right)
	$ holds. Suppose that $x(\tvar_0) \in\mathcal{X}$.
%	 and that there is for each $j \in \mathbb{N}_0$ an $\ivar{j} \in \left[1,\dots,n_\tpar\right]$, such that $\svar_{j+1} - \svar_j \leq \delta T_{\max}\left(\gamma_\ivar{j},L_\ivar{j}+\frac{\epsilon_\ivar{j}}{2}\right)$.  Proposition~\ref{prop_hybrid} thus implies
%	for $\svar_j \leq t \leq \svar_{j+1}$ with $\Lambda_\ivar{j} = L_\ivar{j}+\frac{\epsilon_\ivar{j}}{2}$ that \eqref{eq_set_dec} holds.
	%	\begin{equation}
	%	\label{eq_V_dec_set}
	%	\begin{split}
	%	&U_\ivar{j}(\xi(t,j+1))	\\
	%	\leq&  e^{ -\epsilon_\ivar{j} (t-\svar_j)}V(\xi(\tvar_j)) +\maxvar  \int_{\svar_j}^{t}e^{-\epsilon_\refer (t-\tau)} \alpha_w\left(\abs{w(\tau)}\right) d\tau,
	%	\end{split}
	%	\end{equation}
	%	where $U_\ivar{j}(\xi)$ is the function according to \eqref{eq_def_u} for the parameters $\gamma_\ivar{j}$ and $\Lambda_\ivar{j}$, holds for $\maxvar$ according to \eqref{eq_def_maxvar}. 
	
	Now, we show by induction, that 
	\begin{equation}
	\label{eq_ref_loc_ind}
		\begin{split}
			&V(x(t,j))\\
			\leq& c_w + e^{-\bar \epsilon t} \min\left\lbrace\max\left\lbrace\left(V(x(0,0)) - c_w\right),0 \right\rbrace,c_{\max}-c_w\right\rbrace
		\end{split}
	\end{equation}	
	holds with $\bar\epsilon = \min\left\lbrace\epsilon_1,\epsilon_\refer\right\rbrace$ for all $(t,j)\in \text{dom}~\xi$. It trivially holds for $t = j = 0$. Further suppose it holds  for all $\tvar_j$ with $j \leq \barj$ for some $\barj \in \mathbb{N}$. 
	
	
	We can conclude from the modified version of Algorithm~\ref{algo_trig_window} that either \eqref{eq_dec_gen_loc} and \eqref{eq_bound_aux_loc} hold for $\barj$, some $\ivar{\barj}\in\left\lbrace 2,\dots,n_\tpar\right\rbrace$\MH{Is this the better way to write the set?} and $\svar_\barj \leq t \leq \svar_{\barj+1}$ or that $\svar_{\barj+1} = \svar_{\barj} + T_{\max}(\gamma_1,L_1+\frac{\epsilon_1}{2})$.
	
	In the former case, \eqref{eq_dec_gen_loc} implies since $C(x(\tvar_j),\eta(\tvar_j)) \leq c_{\max}$ that \eqref{eq_bound_U_loc} holds for $\barj$ with $\epsilon = \epsilon_{i_\barj}$. Thus, it follows in this case from Proposition~\ref{prop_hybrid_loc} and the modified version of Algorithm~\ref{algo_trig_window} that \eqref{eq_cond_dec} holds for $\barj$ and $\svar_\barj \leq t \leq \svar_{\barj+1}$. We obtain due to the update of $\eta$ according to \eqref{eq_S_ref} and the definition of $C(x,\eta)$ in \eqref{eq_ref_C_loc} that 
	\begin{equation}
	\label{eq_ref_loc_C}
	\begin{split}
	&C(x(\tvar_\barj),\eta(\tvar_\barj))
	\leq c_w + \eta(\tvar_{\barj})\\
	\leq&c_w +  e^{-\epsilon_\refer \svar_\barj} \min\left\lbrace\max\left\lbrace\left(V(x(0,0)) - c_w\right),0 \right\rbrace,c_{\max}-c_w\right\rbrace
	\end{split}
	\end{equation}
	Plugging \eqref{eq_ref_loc_C} in \eqref{eq_cond_dec}, we can conclude that \eqref{eq_ref_loc_ind} holds in this case for $\barj+1$ and $\svar_\barj \leq t \leq \svar_{\barj+1}$.
	
	In the other case, i.e., if $\svar_{\barj+1} = \svar_{\barj} + T_{\max}(\gamma_1,L_1+\frac{\epsilon_1}{2})$, we observe that \eqref{eq_bound_U_loc} holds for $\epsilon = \epsilon_1$ since $V(x(\tvar_\barj)) \leq c_{\max}$, $\frac{\alpha_w\left(\abs{\bar w}\right)}{\epsilon} \leq c_w \leq c_{\max}$ and $e^{-\epsilon_1 \auxvar(\tvar_\barj^+)} \leq 1$. Thus, we can use in this case Proposition~\ref{prop_hybrid_loc} and obtain that 
	\begin{equation}
	\label{eq_ref_eps1_loc}
	\begin{split}
	V(x(t,\barj+1)) 
	\leq&	e^{ -\epsilon_1 (t-\svar_\barj)}V(x(\tvar_\barj))\\
	& + \frac{\alpha_w\left(\abs{\bar w}\right)}{\epsilon_1} \left(1-e^{-\epsilon_1(t-\svar_\barj)}\right)
	\end{split}
	\end{equation} 
	holds for $\svar_\barj \leq t \leq \svar_{\barj+1}$. Plugging \eqref{eq_ref_loc_ind} for $(t,j) = \tvar_\barj$ into \eqref{eq_ref_eps1_loc}, we obtain 
	\begin{equation}
	\begin{split}
	&V(x(t,\barj+1))\\ 
	\leq&	e^{ -\epsilon_1 (t-\svar_\barj)}\left(c_w + e^{-\bar \epsilon t} \min\left\lbrace\max\left\lbrace\left(V(x(0,0)) - c_w\right),0 \right\rbrace,c_{\max}-c_w\right\rbrace\right)\\
	&+ \frac{\alpha_w\left(\abs{\bar w}\right)}{\epsilon_1} \left(1-e^{-\epsilon_1(t-\svar_\barj)}\right)\\
	\leq& e^{ -\epsilon_1 (t-\svar_\barj)}\min \left\lbrace c_w + e^{-\bar\epsilon \svar_\barj} \max \left\lbrace V(x(0,0)),\abs{\eta(0,0)} \right\rbrace, c_{\max}-c_w \right\rbrace\\
	&+ c_w \left(1-e^{-\epsilon_1(t-\svar_\barj)}\right)\\
	\leq& c_w +  e^{-\epsilon_\refer \svar_\barj} \min\left\lbrace\max\left\lbrace\left(V(x(0,0)) - c_w\right),0 \right\rbrace,c_{\max}-c_w\right\rbrace
	\end{split}
	\end{equation}
	\MH{Seems this violates the page margin...}
	for $\svar_\barj\leq t \leq \svar_{\barj+1}$. Thus \eqref{eq_ref_loc_ind} holds in both cases  also for $\tvar_{\barj+1}$ and hence by induction for all $(t,j) \in\text{dom}~\xi$. RAS of $\mathcal{R}$ follows immediately from \eqref{eq_ref_loc_ind} and $t \geq \frac{t+j t_{\min}}{2}$ which implies that we can chose
	\begin{equation*}
	\begin{split}
	&\beta\left(\abs{\begin{bmatrix}
		x(0,0)\\
		e(0,0)\\
		\eta(0,0)
		\end{bmatrix}},t, j\right)\\
	=& e^{-\bar \epsilon \left(\frac{t+jt_{\min}}{2}\right)} \max \left\lbrace \overline{\alpha}_V \abs{\begin{bmatrix}
		x(0,0)\\
		e(0,0)\\
		\eta(0,0)
		\end{bmatrix}}, \abs{\begin{bmatrix}
		x(0,0)\\
		e(0,0)\\
		\eta(0,0)
		\end{bmatrix}} \right\rbrace.
	\end{split}			 	
	\end{equation*}
	\hfill\hfill\qed

==> proof_theo_set.tex <==
%
\subsubsection{Proof of Theorem~\ref{theo_set}}
\label{proof_theo_set}
	Similar as in the proof of Theorem~\ref{prop_fir}, we obtain that 		
	$t_{\min} \leq \svar_{j+1} - \svar_j \leq t_{\max} \coloneqq \underset{i \in \left[1,\dots,n_\tpar\right]}{\max} \delta T_{\max}\left(\gamma_i,L_i+\frac{\epsilon_i}{2}\right)
	$ holds and that there is for each $j \in \mathbb{N}_0$ an $\ivar{j} \in \left[1,\dots,n_\tpar\right]$, such that $\svar_{j+1} - \svar_j \leq \delta T_{\max}\left(\gamma_\ivar{j},L_\ivar{j}+\frac{\epsilon_\ivar{j}}{2}\right)$.  Proposition~\ref{prop_hybrid} thus implies
	for $\svar_j \leq t \leq \svar_{j+1}$ with $\Lambda_\ivar{j} = L_\ivar{j}+\frac{\epsilon_\ivar{j}}{2}$ that \eqref{eq_set_dec} holds.
	%
	%
	%
	%
	%
	%
	%
	%
	
	Now, we show by induction, that 
	\begin{equation}
	\label{eq_set_ind_res}
	V(x(t,j))\leq c_w + e^{-\bar\epsilon t} \max\left\lbrace\left(V(x(0,0) - c_w)\right),0\right\rbrace
	\end{equation}	
	holds with $\bar\epsilon = \min\left\lbrace\epsilon_1,\epsilon_\refer\right\rbrace$ for all $(t,j)\in \text{dom}~\xi$. It trivially holds for $(t,j) = (0,0)$. Further suppose it holds  for all $\tvar_j$ with $j \leq \barj$ for some $\barj \in \mathbb{N}$. 
	
	If $\svar_{\barj+1}-\svar_\barj \leq T_{\max}\left(\gamma_\ivar{\barj},L_\ivar{\barj}-\frac{\epsilon_\ivar{\barj}}{2}\right)$ for some $\ivar{\barj}\in\left\lbrace 2,\dots,n_\tpar\right\rbrace$, then we can conclude from the modified version of Algorithm~\ref{algo_trig_window} that \eqref{eq_set_bound_ref} holds for $\svar_\barj\leq t \leq \svar_{\barj+1}$ and $\ivar{j} = \ivar{\barj}$ and thus with \eqref{eq_set_dec} that
	\begin{equation}
	\label{eq_set_V1}
	\begin{split}
	V(x(t,\barj+1)) \leq& V_\refer(t,x(0,0))\\
	=& c_w + e^{-\epsilon_\refer t} \max\left\lbrace\left(V(x(0,0) - c_w)\right),0\right\rbrace.
	\end{split}		 
	\end{equation} 
	
	Otherwise, the modified algorithm uses the fall-back strategy, and hence $\svar_{\barj+1}-\svar_\barj \leq T_{\max}\left(\gamma_1,L_1-\frac{\epsilon_1}{2}\right)$. In this case, it follows from \eqref{eq_set_dec} for $\svar_\barj\leq t\leq\svar_{\barj+1}$ that
	\begin{equation}
	\label{eq_set_V2}
	\begin{split}
	&\phantom{\leq}~V(x(t,j+1))\\
	&\leq e^{-\epsilon_1(t-\svar_\barj)}V(x(\tvar_\barj)) + \frac{\alpha_w(\abs{\bar w}) }{\epsilon_1} \left(1-e^{-\epsilon_1 (t-\svar_j)}\right)\\
	\overset{\eqref{eq_set_ind_res}\text{ for }\tvar_j}&{\leq} c_w + e^{-\bar\epsilon t} \max\left\lbrace\left(V(x(0,0) - c_w)\right),0\right\rbrace
	\end{split}		
	\end{equation}
	Combining \eqref{eq_set_V1} and \eqref{eq_set_V2}, we can conclude that \eqref{eq_set_ind_res} holds for $\svar_{\barj} \leq t \leq \svar_{\barj+1}$ and $\barj+1$ and  thus also for $\tvar_{\barj+1}$. Hence it holds by induction for all $(t,j) \in \text{dom}~\xi$.
	
	To construct the function $\beta$ in Definition~\ref{def_set_stab}, we use that $t \geq \frac{t+j t_{\min}}{2}$, which follows from $t_{j+1} - t_j \geq t_{\min}$ for all $j \in \mathbb{N}_0$. We thus obtain from \eqref{eq_set_ind_res} that \eqref{eq_stab_bound_set} holds with
	\begin{equation*}
	\begin{split}
	&\beta\left(\abs{\begin{bmatrix}
		x(0,0)\\
		e(0,0)\\
		\eta(0,0)
		\end{bmatrix}},t, j\right)\\
	=&e^{-\epsilon_\refer \left(\frac{t+j t_{\min}}{2}\right)}  \max\left\lbrace\left(V(x(0,0) - c_w)\right),0\right\rbrace.
	\end{split}
	\end{equation*} \hfill\hfill\qed
	
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%
	%

==> reference_rpi.tex <==
%
\section{Reference RPI}
We assume in this section that $w(t) \bar w$ for all $t\geq 0$, where $\bar{w} \in \mathbb{R}$ is given. 
\MH{could also use here a more general definition with a compact set $\mathcal{W}$}
\begin{defi}
	RPI-set:
	$\mathcal{V}_\RPI \subseteq \mathbb{R}^{n_x}$ such that $ x(t,j) \in \mathcal{V}_\RPI~\forall t \geq t_{\bar j}, j \geq \bar j$ if $x(t_j) \in \mathcal{V}_\RPI$
\end{defi}
\MH{Think about how to define the RPI-Set: if we are inside at a sampling time, we want to stay inside forever. However, we might go outside again if we enter between sampling times?}
Possible outcomes of the algorithm:

 i) $t-\svar_j \leq T_{\max}(\gamma_1,L_1-\frac{\epsilon_1}{2})$:
 Recall from Proposition~\ref{prop_hybrid} that for $t-\svar_j \leq T_{\max}(\gamma_1,L_1-\frac{\epsilon_1}{2})$
\begin{equation*}
\begin{split}
V(x(\svar,j+1)) \leq&	\exp\left( -\epsilon_1 (t-\svar_j)\right)V(x(\tvar_j))\\
&+ \int_{t_j}^{t} \exp\left( \epsilon_1 (t-\tau)\right)\theta_1^p \norm{w(\tau)}^p d\tau\\
\leq &  \exp\left( -\epsilon_1 (t-\svar_j)\right)V(x(\tvar_j))\\
 &+ \frac{\theta_1^p w_{\max}^p }{\epsilon_1} \left(1-\exp\left(-\epsilon_1 (t-\svar_j)\right)\right).
\end{split}
\end{equation*}
holds. 

Now suppose that $\mathcal{V}_\RPI = \left\lbrace x | V(x) \leq c_\RPI \coloneqq \frac{\theta_1^P w_{\max}^p}{\epsilon_1} \right\rbrace$. If $V(x(\tvar_j)) \in \mathcal{V}_\RPI$, then 
\begin{equation*}
	V(x(\svar,j+1)) \leq \frac{\theta_1^p w_{\max}^p }{\epsilon_1}
\end{equation*}
and thus $x(t,j+1) \in \mathcal{V}_\RPI$ for all $t_j \leq t \leq t_j+T_{\max}(\gamma_1,L_1-\frac{\epsilon_1}{2})$. Otherwise, 
\begin{equation}
	\begin{split}
		&V(x(t,j))\\
		 \leq& \frac{\theta_1^p w_{\max}^p }{\epsilon_1} + \exp\left(-\epsilon_1\left(t-t_j\right)\right) \left(V(x(s_j)) -  \frac{\theta_1^p w_{\max}^p }{\epsilon_1}\right)
	\end{split}
\end{equation}
which implies exponential convergence. 

ii) $0 \leq t-\svar_j \leq T_{\max}(\gamma_i,L_i-\frac{\epsilon_i}{2})$ for some $i\in\left\lbrace 1,\dots,n_\tpar\right\rbrace$:
In this case it holds that
\begin{equation*}
\begin{split}
	V(x(t,j)) \leq& \exp\left(-\epsilon_i \left(t-\svar_j\right)\right) V(x(t_j))\\
	 &+ \int_{t_j}^{t} \exp\left( \epsilon_i (t-\tau)\right)\theta_i^p \norm{w(\tau)}^p d\tau\\
	 \leq &  \exp\left(-\epsilon_i \left(t-\svar_j\right)\right) V(x(t_j)\\
	  &+ \frac{\theta_i^p w_{\max}^p }{\epsilon_1} \left(1-\exp\left(-\epsilon_i (t-\svar_j)\right)\right)
\end{split}	
\end{equation*}

We want that $V(x(t,j)) \leq V_\refer(t,j) \coloneqq \exp\left(-\epsilon_\refer t \right) V(x_0) + c_\RPI $. This is the case if 

\begin{equation}
	\begin{split}
	&\exp\left(-\epsilon_i \left(t-\svar_j\right)\right) V(x(t_j)\\
	&+ \frac{\theta_i^p w_{\max}^p }{\epsilon_i} \left(1-\exp\left(-\epsilon_i (t-\svar_j)\right)\right)\\
	\leq & \exp\left(-\epsilon_\refer t \right) V(x_0) + c_\RPI 
	\end{split}
\end{equation}

\MH{The following is only valid if $-\epsilon_i + \epsilon_\refer > 0$}
Now suppose the algorithm choses $\svar_{j+1} - \svar_j$ such that 
\begin{equation*}
\begin{split}
	&\svar_{j+1} - \svar_j\\
	 \leq& \frac{\log\left(\exp\left(-\epsilon_\refer t_j \right) V(x_0)+ c_\RPI -\frac{\theta_i^p w_{\max}^p}{\epsilon_i}\right)}{-\epsilon_i - \epsilon_\refer} \\
	 &-  \frac{\log \left(V(x(t_j))- \frac{\theta_i^pw_{\max}^p}{\epsilon_i}\right)}{-\epsilon_i - \epsilon_\refer},
\end{split}
\end{equation*}
which implies
\begin{equation*}
	\begin{split}
		&\exp\left(\left(-\epsilon_i+\epsilon_\refer\right)  \left(\svar_{j+1} - \svar_j \right)\right) \left(V(x(t_j))- \frac{\theta_i^pw_{\max}^p}{\epsilon_i}\right)\\
		 \leq& \exp\left(-\epsilon_\refer t_j \right) V(x_0)+ c_\RPI -\frac{\theta_i^p w_{\max}^p}{\epsilon_i}
	\end{split}
\end{equation*}
and thus
\begin{equation*}
	\begin{split}
		& \exp\left(-\epsilon_i  \left(\svar_{j+1} - \svar_j \right)\right) \left(V(x(t_j))- \frac{\theta_i^pw_{\max}^p}{\epsilon_i}\right)\\
		\leq & \exp\left(-\epsilon_\refer \left(\svar_{j+1} - \svar_j \right) \right) \left( \exp\left(-\epsilon_\refer t_j \right) V(x_0)+ c_\RPI -\frac{\theta_i^p w_{\max}^p}{\epsilon_i} \right)
	\end{split}
\end{equation*}
